Incremental Non-Rigid Structure-from-Motion with Unknown Focal Length

The perspective camera and the isometric surface prior have recently gathered increased attention for Non-Rigid Structure-from-Motion (NRSfM). Despite the recent progress, several challenges remain, particularly the computational complexity and the unknown camera focal length. In this paper we present a method for incremental Non-Rigid Structure-from-Motion (NRSfM) with the perspective camera model and the isometric surface prior with unknown focal length. In the template-based case, we provide a method to estimate four parameters of the camera intrinsics. For the template-less scenario of NRSfM, we propose a method to upgrade reconstructions obtained for one focal length to another based on local rigidity and the so-called Maximum Depth Heuristics (MDH). On its basis we propose a method to simultaneously recover the focal length and the non-rigid shapes. We further solve the problem of incorporating a large number of points and adding more views in MDH-based NRSfM and efficiently solve them with Second-Order Cone Programming (SOCP). This does not require any shape initialization and produces results orders of times faster than many methods. We provide evaluations on standard sequences with ground-truth and qualitative reconstructions on challenging YouTube videos. These evaluations show that our method performs better in both speed and accuracy than the state of the art.

==> tex/body.tex <==
%
% Compile:
%   - 'paper_for_review.tex', or
%   - 'paper_final.tex'.
%
% Please see README.txt
%

%%%%%%%%% PREAMBLE
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{result}[theorem]{Result}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% \renewcommand\Authands{, }

% for tables
\newcolumntype{Y}{>{\centering\arraybackslash}X}

% ToDo
\newcommand\todo[1]{\textcolor{red}{TODO: {#1}}}
\newcommand\tp[1]{\textcolor{blue}{Thomas: {#1}}}
\newcommand\dp[1]{\textcolor{green}{Danda: {#1}}}
\newcommand\ac[1]{\textcolor{magenta}{Ajad: {#1}}}
\newcommand\lv[1]{\textcolor{red}{Luc: {#1}}}

\newcommand{\myparagraph}[1]{\vspace{0.5em}\noindent\textbf{#1}}
\usepackage{amsmath}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

\begin{document}

%%%%%%%%% TITLE
\input{tex/title.tex}


%%%%%%%%% ABSTRACT
\begin{abstract}
abstract...
\end{abstract}
%
% Acknowledgements
%
% \blfootnote{\textbf{Acknowledgements.} This project has received funding from the European Union’s Horizon 2020 research and innovation programme, and European Research Council project VarCity, under grant agreements No. 637221 and 273940, respectively.}


%%%%%%%%% COPYRIGHT NOTICE
% \fancyhead{}
% \fancyfoot{}
% % \lfoot{\vspace{-12pt} \scriptsize \textit{This is the author's version of a paper published in CVPR 2017. The final publication is available at \href{http://link.springer.com/}{link.springer.com}. \textcopyright Springer International Publishing AG, Switzerland 2016}}
% \lfoot{\vspace{-12pt} \scriptsize \textit{To appear in the Proc. of the IEEE Conference on Computer Vision and Pattern Recognition. (CVPR), Honolulu, Hawaii, USA, July 2017.
% %
% \noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
% %
% \textcopyright 2017 IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.}}
% % \setlength{\headrulewidth}{0pt}
% \thispagestyle{fancy}
% %
% %


%%%%%%%%% BODY TEXT
% intro
\newpage
\input{tex/introduction.tex}
\newpage
% method
\input{tex/method.tex}

% results
\input{tex/results.tex}
\input{tex/conclusion.tex}

%%%%%%%%% REFERENCE
{\small
\bibliographystyle{ieee}
\bibliography{egbib}
}

\end{document}

